Know Your RAG: Dataset Taxonomy and Generation Strategies for Evaluating RAG Systems

Retrieval Augmented Generation (RAG) systems are a widespread application of Large Language Models (LLMs) in the industry. While many tools exist empowering developers to build their own systems, measuring their performance locally, with datasets reflective of the system's use cases, is a technological challenge. Solutions to this problem range from non-specific and cheap (most public datasets) to specific and costly (generating data from local documents). In this paper, we show that using public question and answer (Q&A) datasets to assess retrieval performance can lead to non-optimal systems design, and that common tools for RAG dataset generation can lead to unbalanced data. We propose solutions to these issues based on the characterization of RAG datasets through labels and through label-targeted data generation. Finally, we show that fine-tuned small LLMs can efficiently generate Q&A datasets. We believe that these observations are invaluable to the know-your-data step of RAG systems development.

==> appendices/experiments_old.tex <==
\section{Retrieval Experiments}
\label{appendix:experiments}

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 

\multirow{4}{*}{\hotpotqa} & Inclusive & 0.906 & 0.904 & 0.942 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.890 & 0.878 & \textit{0.924 (-0.076)} & 0.10\\ 
 & \factsingle & 0.891 & 0.897 & 0.930 & 0.10\\ 
 & \summary & 1.000 & 1.000 & \textbf{1.000} & 0.50\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.752 & 0.719 & 0.804 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.708 & 0.706 & \textit{0.784 (-0.051)} & 0.20\\ 
 & \factsingle & 0.790 & 0.770 & \textbf{0.835} & 0.05\\ 
 & \summary & 0.777 & 0.696 & 0.820 & 0.05\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.686 & 0.464 & \textit{0.686 (-0.033)} & 0.00\\  \cline{2-6} 
 & \reasoning & 0.690 & 0.434 & 0.690 & 0.00\\ 
 & \factsingle & 0.705 & 0.493 & 0.705 & 0.00\\ 
 & \summary & 0.719 & 0.436 & \textbf{0.719} & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.249 & 0.494 & 0.500 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.194 & 0.379 & \textit{0.379 (-0.161)} & 1.00\\ 
 & \factsingle & 0.262 & 0.533 & \textbf{0.540} & 0.50\\ 
 & \summary & 0.294 & 0.433 & 0.465 & 0.20\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.949 & 0.895 & \textit{0.935 (-0.052)} & 0.05\\  \cline{2-6} 
 & \reasoning & 0.947 & 0.885 & 0.947 & 0.00\\ 
 & \factsingle & 0.987 & 0.952 & \textbf{0.987} & 0.00\\ 
 & \summary & 0.985 & 0.959 & 0.985 & 0.00\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.776 & 0.831 & 0.871 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.757 & 0.671 & \textit{0.789 (-0.104)} & 0.10\\ 
 & \factsingle & 0.818 & 0.852 & \textbf{0.893} & 0.10\\ 
 & \summary & 0.834 & 0.751 & 0.834 & 0.00\\ 
 
\end{tabular} 
\caption{\label{table:retrieval_1}
Embedding model: \texttt{bge-small-en-v1.5}; Rerank: False} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 


\multirow{4}{*}{\hotpotqa} & Inclusive & 0.933 & 0.946 & 0.965 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.907 & 0.919 & \textit{0.948 (-0.052)} & 0.10\\ 
 & \factsingle & 0.926 & 0.938 & 0.954 & 0.10\\ 
 & \summary & 1.000 & 1.000 & \textbf{1.000} & 0.10\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.790 & 0.780 & 0.795 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.749 & 0.763 & \textit{0.749 (-0.093)} & 0.00\\ 
 & \factsingle & 0.825 & 0.822 & \textbf{0.842} & 0.20\\ 
 & \summary & 0.822 & 0.788 & 0.822 & 0.00\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.695 & 0.580 & 0.695 & 0.00\\  \cline{2-6} 
 & \reasoning & 0.673 & 0.562 & \textit{0.687 (-0.056)} & 0.10\\ 
 & \factsingle & 0.723 & 0.614 & \textbf{0.743} & 0.05\\ 
 & \summary & 0.715 & 0.560 & 0.715 & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.300 & 0.461 & 0.463 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.210 & 0.315 & \textit{0.323 (-0.178)} & 0.20\\ 
 & \factsingle & 0.320 & 0.498 & \textbf{0.501} & 0.50\\ 
 & \summary & 0.302 & 0.384 & 0.388 & 0.50\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.892 & 0.908 & 0.896 & 0.05\\  \cline{2-6} 
 & \reasoning & 0.887 & 0.907 & \textit{0.887 (-0.078)} & 0.00\\ 
 & \factsingle & 0.941 & 0.961 & 0.965 & 0.50\\ 
 & \summary & 0.965 & 0.977 & \textbf{0.965} & 0.00\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.659 & 0.828 & 0.830 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.618 & 0.757 & \textit{0.763 (-0.106)} & 0.20\\ 
 & \factsingle & 0.717 & 0.867 & \textbf{0.869} & 0.50\\ 
 & \summary & 0.716 & 0.834 & 0.852 & 0.20\\ 
 
\end{tabular} 
\caption{\label{table:retrieval_2}
Embedding model: \texttt{bge-small-en-v1.5}; Re-ranking model: \texttt{BGE-base}} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 


\multirow{4}{*}{\hotpotqa} & Inclusive & 0.830 & 0.904 & 0.929 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.767 & 0.878 & \textit{0.907 (-0.093)} & 0.10\\ 
 & \factsingle & 0.813 & 0.897 & 0.914 & 0.10\\ 
 & \summary & 0.818 & 1.000 & \textbf{1.000} & 0.10\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.697 & 0.719 & 0.799 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.661 & 0.706 & \textit{0.781 (-0.053)} & 0.20\\ 
 & \factsingle & 0.740 & 0.770 & \textbf{0.834} & 0.10\\ 
 & \summary & 0.711 & 0.696 & 0.801 & 0.05\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.625 & 0.464 & 0.625 & 0.00\\  \cline{2-6} 
 & \reasoning & 0.623 & 0.434 & \textit{0.623 (-0.018)} & 0.00\\ 
 & \factsingle & 0.641 & 0.493 & \textbf{0.641} & 0.00\\ 
 & \summary & 0.640 & 0.436 & 0.640 & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.186 & 0.494 & 0.496 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.177 & 0.379 & \textit{0.379 (-0.156)} & 1.00\\ 
 & \factsingle & 0.195 & 0.533 & \textbf{0.535} & 0.50\\ 
 & \summary & 0.229 & 0.433 & 0.441 & 0.50\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.886 & 0.895 & \textit{0.902 (-0.075)} & 0.50\\  \cline{2-6} 
 & \reasoning & 0.877 & 0.885 & 0.922 & 0.10\\ 
 & \factsingle & 0.944 & 0.952 & 0.969 & 0.05\\ 
 & \summary & 0.935 & 0.959 & \textbf{0.977} & 0.10\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.773 & 0.831 & 0.878 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.743 & 0.671 & \textit{0.803 (-0.096)} & 0.10\\ 
 & \factsingle & 0.816 & 0.852 & \textbf{0.899} & 0.10\\ 
 & \summary & 0.852 & 0.751 & 0.852 & 0.05\\ 
 
\end{tabular} 
\caption{\label{table:retrieval_3}
Embedding model: \texttt{all-minilm-l6-v2}; Rerank: False} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 


\multirow{4}{*}{\hotpotqa} & Inclusive & 0.881 & 0.946 & 0.959 & 0.10\\  \cline{2-6} 
 & \reasoning & 0.814 & 0.919 & \textit{0.814 (-0.186)} & 0.00\\ 
 & \factsingle & 0.868 & 0.938 & 0.868 & 0.00\\ 
 & \summary & 1.000 & 1.000 & \textbf{1.000} & 0.50\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.773 & 0.780 & 0.804 & 0.20\\  \cline{2-6} 
 & \reasoning & 0.724 & 0.763 & \textit{0.784 (-0.051)} & 0.50\\ 
 & \factsingle & 0.814 & 0.822 & 0.814 & 0.00\\ 
 & \summary & 0.810 & 0.788 & \textbf{0.835} & 0.20\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.668 & 0.580 & 0.668 & 0.00\\  \cline{2-6} 
 & \reasoning & 0.630 & 0.562 & 0.658 & 0.05\\ 
 & \factsingle & 0.697 & 0.614 & \textbf{0.722} & 0.05\\ 
 & \summary & 0.655 & 0.560 & \textit{0.655 (-0.067)} & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.239 & 0.461 & 0.462 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.218 & 0.315 & \textit{0.331 (-0.169)} & 0.10\\ 
 & \factsingle & 0.254 & 0.498 & \textbf{0.500} & 0.50\\ 
 & \summary & 0.229 & 0.384 & 0.388 & 0.10\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.878 & 0.908 & \textit{0.899 (-0.078)} & 0.05\\  \cline{2-6} 
 & \reasoning & 0.869 & 0.907 & 0.913 & 0.20\\ 
 & \factsingle & 0.938 & 0.961 & 0.938 & 0.00\\ 
 & \summary & 0.956 & 0.977 & \textbf{0.977} & 1.00\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.678 & 0.828 & 0.830 & 0.50\\  \cline{2-6} 
 & \reasoning & 0.625 & 0.757 & 0.757 & 0.50\\ 
 & \factsingle & 0.738 & 0.867 & \textit{0.738 (-0.108)} & 0.00\\ 
 & \summary & 0.722 & 0.834 & \textbf{0.846} & 0.10\\ 
 
\end{tabular} 
\caption{\label{table:retrieval_4}
Embedding model: \texttt{all-minilm-l6-v2}; Re-ranking model: \texttt{BGE-base}} 
\end{table*}

\Cref{table:retrieval_1,,table:retrieval_2,,table:retrieval_3,,table:retrieval_4} show the dependence of the retrieval performance on proposed taxonomy. We quantify the results with the use of the Recall@5 metric. \Cref{table:retrieval_1,,table:retrieval_2} employ the embedding model \texttt{bge-small-en-v1.5}, with the latter also re-ranking the retrieval results with the \texttt{bge-base} re-ranker. \Cref{table:retrieval_3,,table:retrieval_4} employ the embedding model \texttt{all-minilm-l6-v2}, with the latter also re-ranking the retrieval results with the \texttt{bge-base} re-ranker. 
We do not show the results for the \unanswerable~label as that is not a label of interest for our study. However, these questions are included in the ``Inclusive'' evaluation, which reflects the standard use of these datasets by the public. For this reason, the retrieval performance of the ``Inclusive'' evaluation can be lower than any of the displayed individual labels. The results for the \hotpotqa~ \summary~label are statistically limited by the number of Q\&As present in the analysed dataset after labelling -- we leave them in the results tables for completeness.

% \clearpage

==> tables/data_composition.tex <==
\begin{table*}[t]
    
    
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} lrrrr}
        \toprule
\textbf{Dataset} & \textbf{fact\_single} & \textbf{reasoning} & \textbf{summary} & \textbf{unanswerable} \\
        \midrule
        
\textbf{HotpotQA} & 42.9\% & 3.4\% & 0.2\% & \textbf{53.4\%}\\ 
\textbf{MS MARCO} & \textbf{41.8\%} & 8.8\% & 27.9\% & 21.5\%\\ 
\textbf{NaturalQ} & \textbf{68.9\%} & 5.6\% & 9.9\% & 15.6\%\\ 
\textbf{NewsQA} & \textbf{83.0\%} & 1.8\% & 3.6\% & 11.7\%\\ 
\textbf{PubMedQA} & 15.8\% & \textbf{53.9\%} & 9.9\% & 20.3\%\\ 
\textbf{SQuAD2} & \textbf{68.2\%} & 2.2\% & 2.4\% & 27.1\%\\ 

        
        \bottomrule
    \end{tabular*}
    \caption{\label{table:data_comp}
    Datasets considered in the study.}
\end{table*}

==> tables/datasets.tex <==
\begin{table}[t]
    
    
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} lrr}
        \toprule
        \textbf{Dataset} & \textbf{Label Q\&As} & \textbf{Contexts} \\
        \midrule

        
        \textbf{SQuAD2} & 6910 & 19029 \\

        \textbf{NewsQA} & 6890 & 89481 \\

        \textbf{PubMedQA} & 6847 & 61243 \\

        \textbf{HotpotQA} & 5000 & 65489 \\

        \textbf{MS MARCO} & 4972 & 808712 \\

        \textbf{NaturalQ} & 5000 & 111388 \\

        
        \bottomrule
    \end{tabular*}
    \caption{\label{table:datasets}
    Datasets considered in the study.}
\end{table}

==> tables/retrieval_results.tex <==

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 

\multirow{4}{*}{\hotpotqa} & Inclusive & 0.906 & 0.904 & 0.942 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.890 & 0.878 & \textit{0.924 (-0.076)} & 0.10\\ 
 & \factsingle{} & 0.891 & 0.897 & 0.930 & 0.10\\ 
 & \summary{} & 1.000 & 1.000 & \textbf{1.000} & 0.50\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.752 & 0.719 & 0.804 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.708 & 0.706 & \textit{0.784 (-0.051)} & 0.20\\ 
 & \factsingle{} & 0.790 & 0.770 & \textbf{0.835} & 0.05\\ 
 & \summary{} & 0.777 & 0.696 & 0.820 & 0.05\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.686 & 0.464 & \textit{0.686 (-0.033)} & 0.00\\  \cline{2-6} 
 & \reasoning{} & 0.690 & 0.434 & 0.690 & 0.00\\ 
 & \factsingle{} & 0.705 & 0.493 & 0.705 & 0.00\\ 
 & \summary{} & 0.719 & 0.436 & \textbf{0.719} & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.249 & 0.494 & 0.500 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.194 & 0.379 & \textit{0.379 (-0.161)} & 1.00\\ 
 & \factsingle{} & 0.262 & 0.533 & \textbf{0.540} & 0.50\\ 
 & \summary{} & 0.294 & 0.433 & 0.465 & 0.20\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.949 & 0.895 & \textit{0.935 (-0.052)} & 0.05\\  \cline{2-6} 
 & \reasoning{} & 0.947 & 0.885 & 0.947 & 0.00\\ 
 & \factsingle{} & 0.987 & 0.952 & \textbf{0.987} & 0.00\\ 
 & \summary{} & 0.985 & 0.959 & 0.985 & 0.00\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.776 & 0.831 & 0.871 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.757 & 0.671 & \textit{0.789 (-0.104)} & 0.10\\ 
 & \factsingle{} & 0.818 & 0.852 & \textbf{0.893} & 0.10\\ 
 & \summary{} & 0.834 & 0.751 & 0.834 & 0.00\\ 
 
\end{tabular} 
\caption{Model: bge-small-en-v1.5; Rerank: False; Recall@: 5} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 


\multirow{4}{*}{\hotpotqa} & Inclusive & 0.933 & 0.946 & 0.965 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.907 & 0.919 & \textit{0.948 (-0.052)} & 0.10\\ 
 & \factsingle{} & 0.926 & 0.938 & 0.954 & 0.10\\ 
 & \summary{} & 1.000 & 1.000 & \textbf{1.000} & 0.10\\ 

\hline \hline 

\multirow{4}{*}{MSMarco} & Inclusive & 0.790 & 0.780 & 0.795 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.749 & 0.763 & \textit{0.749 (-0.093)} & 0.00\\ 
 & \factsingle{} & 0.825 & 0.822 & \textbf{0.842} & 0.20\\ 
 & \summary{} & 0.822 & 0.788 & 0.822 & 0.00\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.695 & 0.580 & 0.695 & 0.00\\  \cline{2-6} 
 & \reasoning{} & 0.673 & 0.562 & \textit{0.687 (-0.056)} & 0.10\\ 
 & \factsingle{} & 0.723 & 0.614 & \textbf{0.743} & 0.05\\ 
 & \summary{} & 0.715 & 0.560 & 0.715 & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.300 & 0.461 & 0.463 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.210 & 0.315 & \textit{0.323 (-0.178)} & 0.20\\ 
 & \factsingle{} & 0.320 & 0.498 & \textbf{0.501} & 0.50\\ 
 & \summary{} & 0.302 & 0.384 & 0.388 & 0.50\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.892 & 0.908 & 0.896 & 0.05\\  \cline{2-6} 
 & \reasoning{} & 0.887 & 0.907 & \textit{0.887 (-0.078)} & 0.00\\ 
 & \factsingle{} & 0.941 & 0.961 & 0.965 & 0.50\\ 
 & \summary{} & 0.965 & 0.977 & \textbf{0.965} & 0.00\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.659 & 0.828 & 0.830 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.618 & 0.757 & \textit{0.763 (-0.106)} & 0.20\\ 
 & \factsingle{} & 0.717 & 0.867 & \textbf{0.869} & 0.50\\ 
 & \summary{} & 0.716 & 0.834 & 0.852 & 0.20\\ 
 
\end{tabular} 
\caption{Model: bge-small-en-v1.5; Rerank: True; Recall@: 5; Rerank model: bgebase} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 


\multirow{4}{*}{\hotpotqa} & Inclusive & 0.830 & 0.904 & 0.929 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.767 & 0.878 & \textit{0.907 (-0.093)} & 0.10\\ 
 & \factsingle{} & 0.813 & 0.897 & 0.914 & 0.10\\ 
 & \summary{} (*) & 0.818 & 1.000 & \textbf{1.000} & 0.10\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.697 & 0.719 & 0.799 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.661 & 0.706 & \textit{0.781 (-0.053)} & 0.20\\ 
 & \factsingle{} & 0.740 & 0.770 & \textbf{0.834} & 0.10\\ 
 & \summary{} & 0.711 & 0.696 & 0.801 & 0.05\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.625 & 0.464 & 0.625 & 0.00\\  \cline{2-6} 
 & \reasoning{} & 0.623 & 0.434 & \textit{0.623 (-0.018)} & 0.00\\ 
 & \factsingle{} & 0.641 & 0.493 & \textbf{0.641} & 0.00\\ 
 & \summary{} & 0.640 & 0.436 & 0.640 & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.186 & 0.494 & 0.496 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.177 & 0.379 & \textit{0.379 (-0.156)} & 1.00\\ 
 & \factsingle{} & 0.195 & 0.533 & \textbf{0.535} & 0.50\\ 
 & \summary{} & 0.229 & 0.433 & 0.441 & 0.50\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.886 & 0.895 & \textit{0.902 (-0.075)} & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.877 & 0.885 & 0.922 & 0.10\\ 
 & \factsingle{} & 0.944 & 0.952 & 0.969 & 0.05\\ 
 & \summary{} & 0.935 & 0.959 & \textbf{0.977} & 0.10\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.773 & 0.831 & 0.878 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.743 & 0.671 & \textit{0.803 (-0.096)} & 0.10\\ 
 & \factsingle{} & 0.816 & 0.852 & \textbf{0.899} & 0.10\\ 
 & \summary{} & 0.852 & 0.751 & 0.852 & 0.05\\ 
 
\end{tabular} 
\caption{Model: all-minilm-l6-v2; Rerank: False; Recall@: 5} 
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering 
\begin{tabular}{c|c|c|c||c|c}

\textbf{Dataset} & \textbf{Label} & \textbf{Dense} & \textbf{Lexical} & \textbf{Best recall} & \textbf{Best strategy}\\ 

\hline \hline 


\multirow{4}{*}{\hotpotqa} & Inclusive & 0.881 & 0.946 & 0.959 & 0.10\\  \cline{2-6} 
 & \reasoning{} & 0.814 & 0.919 & \textit{0.814 (-0.186)} & 0.00\\ 
 & \factsingle{} & 0.868 & 0.938 & 0.868 & 0.00\\ 
 & \summary{} (*) & 1.000 & 1.000 & \textbf{1.000} & 0.50\\ 

\hline \hline 

\multirow{4}{*}{\msmarco} & Inclusive & 0.773 & 0.780 & 0.804 & 0.20\\  \cline{2-6} 
 & \reasoning{} & 0.724 & 0.763 & \textit{0.784 (-0.051)} & 0.50\\ 
 & \factsingle{} & 0.814 & 0.822 & 0.814 & 0.00\\ 
 & \summary{} & 0.810 & 0.788 & \textbf{0.835} & 0.20\\ 
 
 \hline \hline 
 
\multirow{4}{*}{\naturalq} & Inclusive & 0.668 & 0.580 & 0.668 & 0.00\\  \cline{2-6} 
 & \reasoning{} & 0.630 & 0.562 & 0.658 & 0.05\\ 
 & \factsingle{} & 0.697 & 0.614 & \textbf{0.722} & 0.05\\ 
 & \summary{} & 0.655 & 0.560 & \textit{0.655 (-0.067)} & 0.00\\ 
 
 \hline \hline
 
\multirow{4}{*}{\newsqa} & Inclusive & 0.239 & 0.461 & 0.462 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.218 & 0.315 & \textit{0.331 (-0.169)} & 0.10\\ 
 & \factsingle{} & 0.254 & 0.498 & \textbf{0.500} & 0.50\\ 
 & \summary{} & 0.229 & 0.384 & 0.388 & 0.10\\ 
 
 \hline \hline

\multirow{4}{*}{\pubmedqa} & Inclusive & 0.878 & 0.908 & \textit{0.899 (-0.078)} & 0.05\\  \cline{2-6} 
 & \reasoning{} & 0.869 & 0.907 & 0.913 & 0.20\\ 
 & \factsingle{} & 0.938 & 0.961 & 0.938 & 0.00\\ 
 & \summary{} & 0.956 & 0.977 & \textbf{0.977} & 1.00\\ 

\hline \hline

\multirow{4}{*}{\squad} & Inclusive & 0.678 & 0.828 & 0.830 & 0.50\\  \cline{2-6} 
 & \reasoning{} & 0.625 & 0.757 & 0.757 & 0.50\\ 
 & \factsingle{} & 0.738 & 0.867 & \textit{0.738 (-0.108)} & 0.00\\ 
 & \summary{} & 0.722 & 0.834 & \textbf{0.846} & 0.10\\ 
 
\end{tabular} 
\caption{Model: all-minilm-l6-v2; Rerank: True; Recall@: 5; Rerank model: bgebase} 
\end{table*}
